Bounded Model Checking for Hyperproperties

Hyperproperties are properties of systems that relate multiple computation traces, including security and concurrency properties. This paper introduces a bounded model checking (BMC) algorithm for hyperproperties expressed in HyperLTL, which - to the best of our knowledge - is the first such algorithm. Just as the classic BMC technique for LTL primarily aims at finding bugs, our approach also targets identifying counterexamples. BMC for LTL is reduced to SAT solving, because LTL describes a property via inspecting individual traces. HyperLTL allows explicit and simultaneous quantification over traces and describes properties that involves multiple traces and, hence, our BMC approach naturally reduces to QBF solving. We report on successful and efficient model checking, implemented in a tool called HyperQube, of a rich set of experiments on a variety of case studies, including security, concurrent data structures, path planning for robots, and testing.

==> casestudies.tex <==
\section{Evaluation and Case Studies}

\newcommand{\HyperQube}{\code{HyperQube}\xspace}
\newcommand{\Ocaml}{\code{Ocaml}\xspace}
\newcommand{\select}{\mathit{select}}
\newcommand{\sym}{\mathit{sym}}
\newcommand{\pause}{\mathit{pause}}
\newcommand{\pc}{\mathit{pc}}
\newcommand{\pushRight}{\mathit{pushRight}}
\newcommand{\popLeft}{\mathit{popLeft}}
\newcommand{\history}{\mathit{history}}
\newcommand{\invocations}{\mathit{invocations}}
\newcommand{\response}{\mathit{responses}}
\newcommand{\linearizability}{\mathit{linearizability}}

\newcommand{\NI}{\mathit{NI}}
\newcommand{\terminate}{\mathit{terminate}}
\newcommand{\PIN}{\mathit{PIN}}
\newcommand{\Result}{\mathit{Result}}

\newcommand{\NRR}{\mathit{NRR}}
\newcommand{\NRO}{\mathit{NRO}}

\newcommand{\partyA}{A}
\newcommand{\partyB}{B}
\newcommand{\Act}{\mathit{Act}}
\newcommand{\skipp}{\mathbf{skip}}

\newcommand{\effectiveness}{\mathit{effectiveness}}
\newcommand{\fairnessforA}{\mathit{fairness\ for\ A}}
\newcommand{\fairnessforB}{\mathit{fairness\ for\ B}}

\newcommand{\goal}{\mathit{goal}}

\newcommand{\strategy}{\mathit{strategy}}

\newcommand{\correct}{\mathit{correct}}
\newcommand{\incorrect}{\mathit{incorrect}}

\newcommand{\fair}{\mathit{fair}}


\newcommand{\mut}{\mathit{mut}}
\newcommand{\inputt}{\mathit{input}}
\newcommand{\outputt}{\mathit{output}}



\newcommand{\hpes}{\mathit{halting-pessimistic}}
\newcommand{\hopt}{\mathit{haalting-optimistic}}


\newcommand{\pes}{\textit{pessimistic}}
\newcommand{\opt}{\textit{optimsitic}}
\newcommand{\bpes}{\textit{halting-pes}}
\newcommand{\bopt}{\textit{halting-opt}}
\newcommand{\shortest}{\mathit{shortest\ path}}
\newcommand{\rub}{\mathit{robustness}}


\tzuhan{hi}

In this section, we evaluate our technique using a rich set of case studies 
including verification of symmetry, linearizability, non-interference, and 
non-repudiation. We also used our technique in path planning in robotics as 
well as  test case generation for mutation testing. Our tool \HyperQube works 
as follows. Given a transition relation, we automatically unfold it up to some 
bound $k \geq 0$ using a home-grown tool written in \Ocaml. The unfolded 
transition relation along with the QBF encoding of input HyperLTL formula will 
form a complete QBF instance which will then be fed to the QBF solver 
\code{Quabs}~\cite{ht18}. All experiments in this section are run on an iMac 
desktop with XXX CPU and XXX RAM.

\subsection{Case study 1: Symmetry in the Bakery Algorithm}

We first investigate the symmetry property in Lamport's Bakery 
algorithm for enforcing mutual exclusion in a concurrent program. The 
algorithm works as follows. When a process intends to enter the critical 
section, a ticket with a special number will be drawn by the process. When more 
than one process requests to enter the critical section, the process with 
the smallest ticket number enters first, while other processes wait. In a 
concurrent program, it is also possible that two or more processes hold tickets 
with same number if they drew tickets at the same time. To solve this, while 
ticket comparison is a tie, we let the process with smaller process ID enter the
critical section first and keep others in waiting.

We now consider the symmetry property, where if there is no specific process 
in a program that owns special privilege.
%
We use atomic proposition $\select$ to represent the process 
selected to proceed in the next state, and $\pause$ to indicate if the 
prcoess is not moving. Each process $P_n$ has a program counter denoted by 
$\pc(P_n)$.
%
The symmetry property of the bakery algorithm is the following.
%
For all traces $\pi$, there exists a trace $\pi'$, such that if both traces 
pause together and both select the next process to execute symmetrically, then
the program counter of each process would be completely symmetric as well.
%
For example, for two processes $P_0$ and $P_1$, trace $\pi$ selects $P_0$ \; 
iff \; trace $\pi'$ selects $P_1$, and $\pi$ selects $P_1$ \; iff \; $\pi'$ 
selects $P_0$.
%
Such a scenario is presented as $\sym(\select_{\pi}, \select_{\pi'})$.
%
We now describe the specification as the following HyperLTL formula:

\begin{center}
\centering % used for centering table
\begin{tabular}{ |c|c| } 
\hline
\thead{Symmetry} & \thead{ $\varphi_{\sym} = \forall \pi. \exists\pi'.\ 
\always\Big(\sym(\select_{\pi}, \select_{\pi'}) \land (\pause_{\pi}= 
\pause_{\pi'}) \; \land  $ \\ $\hfill  \big(\pc(P_0)_{\pi} = 
\pc(P_1)_{\pi'}\big) \land \big(\pc(P_1)_{\pi} = \pc(P_0)_{\pi'}\big)\Big)$} \\
\hline
\end{tabular}
\end{center}

Now, observe that the negation of the above formula is:

\begin{center}
\centering % used for centering table
\begin{tabular}{ |c|c| } 
\hline
\thead{$\neg$Symmetry} & \thead{ $\neg \varphi_\sym = \exists \pi.  \forall 
\pi'.\  {\F}\Big( \neg \sym(\select_{\pi}, \select_{\pi'}) \lor  (\pause_{\pi} 
\neq \pause_{\pi'})  \; \lor $ \\ $\hfill(\pc(P_0)_{\pi} \neq \pc(P_1)_{\pi'}) 
\lor (\pc(P_1)_{\pi} \neq \pc(P_0)_{\pi'})\Big)$} \\
\hline
\end{tabular}
\end{center}
%
In this case study, \HyperQube returns SAT, which indicates that there exists a 
trace that satisfy $\neg \varphi_\sym$. 
%
The returned trace represents a witness in the Bakery algorithm that violates symmetry and thus falsifies the original 
formula $\varphi_\sym$. 
%
\textcolor{red}{By analyzing the result with $\pes$ semantics, a observable witness within finite bound is sufficient to infer that all
future observations are consistently indicating the given model does not satisfy original property.}
%
That is, the Bakery algorithm does not satisfy symmetry.


\subsection{Case study 2: Linearizability in SNARK Algorithm}
%
Next, we investigate linearizability property in SNARK algorithm. 
%
Linearizability is a correctness property for concurrent program.
%
In a concurrent system, a $\history$ is a collection of method {\em 
invocations} and {\em response} executed by different threads.  
%
We say that a $\history$ is {\em linearizable}~\cite{hw90}, if there exists a 
sequential order of invocations and responses, such that the responses are 
returned with atomic executions of the whole method.  
%
A concurrent program satisfies linearizability if all possible histories are 
linearizable. In~\cite{bss18}, the authors show that linearizability is a 
hyperproperty of the form $\forall\exists$, where the domain of the universal 
quantifier is over all possible executions of the concurrent data structure and 
the domain of the existential quantifier is over all possible executions of the 
sequential implementation of the data structure. Thus, reasoning 
about linearizability requires our multi-model semantics introduced in 
Section~\ref{sec:prelim}.

The SNARK algorithm~\cite{ddgflmmss04} is a concurrent implementation of a 
double-ended queue data structure.
%
It uses double-compare-and-swap (DCAS) with doubly linked-list that stores 
values in nodes while each node is connected to its two neighbors, $L$ and $R$. 
%
When a modification of data happens, e.g., by invoking \code{pushRight()} or 
\code{popLeft()}, SNARK conducts DCAS by comparing two memory locations to 
decide if such modification is appropriate. 

We define the hyperproperty of linearizability using two different models.
%
Let $\pi_m$ denote the trace variable over the traces of the {\em model} (in 
this case SNARK). This model allows multiple threads to execute each method 
with interleavings.
%
Let $\pi_s$ represents the trace variable over traces of the sequential 
implementation of a double-ended queue (i.e., the specification), where only 
atomic invocations are allowed. 
%
The HyperLTL formula specifying a linearizable program is as follows:   

\begin{center}
\centering % used for centering table
\begin{tabular}{ |c|c| } 
\hline
\thead{Linearizability} & \thead{ $\varphi_{\linearizability} = \forall  
\pi_{m}. \exists \pi_{s}. \ {\always}(\history_{\pi_m} \,
\leftrightarrow \, \history_{\pi_s})$} \\
\hline
\end{tabular}
\end{center}

The negation of the above formula is:

\begin{center}
\centering % used for centering table
\begin{tabular}{ |c|c| } 
\hline
\thead{$\neg$ Linearizability} & \thead{ $\neg \varphi_{\linearizability} = 
\exists \pi_{m}. \forall \pi_{s}. \ {\F}(\history_{\pi_m} 
\not\leftrightarrow \history_{\pi_s})$} \\
\hline
\end{tabular}
\end{center}
%
In this case study, \HyperQube returns SAT, indicating that a witness of 
linearizability violation has been found in SNARK algorithm.
%
The returned trace is a history that cannot be performed when only atomic 
executions are allowed.
%
\textcolor{red}{Consider the resulting trace with $\pes$ semantics, a trace that violates linearizability within bound $k$ 
is not remediable. In other words, finding a witness of linearizability violation within finite observation is enough to draw 
conclusion, such that the given model does not satisfy linearizability property. }
%
The bug we identified by using \HyperQube is the same 
as the one reported in~\cite{ddgflmmss04}.


\subsection{Case study 3: Non-interference in Typed Multi-threaded Programs}
%
We also investigate {\em non-interference} in a multi-threaded 
program with type system.
%
As a security policy, non-interference guarantees that low-security variables 
are independent from the high-security variables, thus, preserving secure 
information flow. 
%
For a concurrent program, a type system classifies each variable as either {\em 
high} or {\em low} security, labeled as {\em high-variable} and { \em 
low-variable}. 
%
Non-interference requires that all information about a high-variable cannot be 
inferred by observing any the value of a low-variable.
%
In this case study, we look at a concurrent system example in~\cite{sv98}, 
which 
contains three threads $\alpha$, $\beta$, and $\omega$. 
%
The variables are assigned with different security level as follows. {\em PIN}, {\em trigger0}, and {\em trigger1} are classified as high-variable, and {\em maintrigger}, {\em mask}, and {\em result} are low-variables. 
%
In a multi-threaded setting, assuming that thread scheduling is fair, the 
program satisfies non-interference, if for all executions, there exists 
another one such that they start from different high-inputs (i.e., the values of 
{\em PIN} are not equal) and at termination point, they are in low-equivalent 
states (i.e., the values of {\em Result} are equal). 
%

Furthermore, in order to search for a witness of non-interference violation in 
bounded time, we also consider the {\em termination bound} introduced in 
Section~\ref{sec:boundedHyperLTL}. 
%
In this particular program, the execution terminates when the low-variable {\em 
MASK} contains value zero. 
%
The corresponding HyperLTL formula is as follows: 

\begin{center}
\centering % used for centering table
\begin{tabular}{ |c|c| } 
\hline
\thead{$\NI$} & \thead{ $\varphi_{\NI} =\forall \pi. \exists \pi'. 
\big(\PIN_\pi 
\neq \PIN_{\pi'}\big) \land \Big((\neg \terminate_{\pi} \lor \neg 
\terminate_{\pi'})$ \\ 
$\hfill \mathcal U \ \big((\terminate_{\pi} \land \terminate_{\pi'}) \land 
(\Result_\pi = \Result_{\pi'}) \big) \Big)\ $} \\
\hline
\end{tabular}
\end{center}
%
where atomic proposition $\terminate$ denotes the terminating state ({\em 
MASK} contains a zero bit) and by abuse of notation $\PIN_\pi$ (respectively, 
$\Result_\pi$) denotes the value of $\PIN$ (respectively, $\Result$) in trace 
$\pi$.
%
The negated formula for BMC is then:
%
%
\begin{center}
\centering % used for centering table
\begin{tabular}{ |c|c| } 
\hline
\thead{$\neg\NI$} & \thead{ $\neg\varphi_{\NI} = \exists \pi. \forall \pi'. 
\big(\PIN_{\pi} \neq \PIN_{\pi'} \big) \rightarrow \Big((\terminate_{\pi} \land \terminate_{\pi'})$ \\
$\hfill \mathcal R\ \big( (\neg \terminate_{\pi} \lor \neg 
\terminate_{\pi'}) \lor  (\Result_{\pi}\neq \Result_{\pi'})\big)\Big)\  $} \\
\hline
\end{tabular}
\end{center}

%
In this case study, \HyperQube returns SAT, indicating that there is a trace we 
can detect the difference of high-variable by observing low variable, that is, 
violating non-interference. 
%
Moreover, by taking terminating bound into consideration, further unrollings 
of transition relation will not affect the result of original model checking 
problem.
%
\textcolor{red}{Take $\hpes$ semantics in to our analysis, a system with halting state is expected to
eventually reach the terminating scenario within finite bound. In this case, $\HyperQube$ spots a violation
together with the halting bit (a predicate {\em halt}), which gives us the infinite inference that a violation
will hold forever. Thus we conclude that the give model does not satisfy non-interference. }
%

\subsection{Case study 4: Fairness in Non-repudiation Protocols}

%
A non-repudiation protocol consists of three parties: a message sender 
($\partyA$), a message receiver ($\partyB$), and a {\em trusted third party} 
$T$. 
%
In a message exchange event, the message receiver should obtain a receipt from 
the sender, named {\em non-repudiation\ of\ origin} ($\NRO$), and the message 
sender should end up having an evidence named {\em non-repudiation of receipt} 
($\NRR$). 
%
A {\em fair} non-repudiation protocol guarantees that two parties can exchange messages fairly without any party being able to deny sending out evidence while having received an evidence. 
%
The three participants can take the following actions: 
%
\begin{align*}
\Act_A & = \{ A \rightarrow B:m,  A \rightarrow T:m , A \rightarrow B:\NRO 
, A \rightarrow T:\NRO , A:\skipp \}\\
%
\Act_B & = \{ B \rightarrow A:\NRR ,  B \rightarrow T:\NRR , B:\skipp \}\\
%
\Act_T & = \{ T \rightarrow A:\NRR ,  T \rightarrow B:\NRO , T:\skipp \}
\end{align*}

We say that a trace is {\em effective} if {\em message}, $\NRR$, and $\NRO$ are 
all received. 
%
Assuming that each party will take turns and take different actions, the fairness of non-repudiation protocol can be presented as hyperproperty as follows. 
%
There exists an {\em effective} trace $\pi$, such that for all other traces 
$\pi'$, if $\partyA$ in both traces always take the same action while $\partyB$ 
behave arbitrarily, or both $\partyB$ take the same action and $\partyA$ behave 
arbitrarily, then for $\pi'$, eventually $\NRR$ gets received by $\partyA$ if 
and only if $\NRO$ gets received by $\partyB$. The complete specification for 
non-repudiation is the following:


% NRP
\begin{center}
\centering % used for centering table
\begin{tabular}{ |c|c| } 
\hline
\thead{Fairness} & \thead[l]{ 
$\varphi_{\fair} = \exists \pi. \forall \pi'.$  $({\F} m_{\pi}) \land ({\F} 
\NRR_{\pi}) \land ({\F} \NRO_{\pi}) \; \land $\\
%
$\hspace{1cm} \Big(({\always} \bigwedge_{a \in \Act_A} a_{\pi} \leftrightarrow 
a_{\pi'} )\ \rightarrow \big(({\F} \NRR_{\pi'}) \leftrightarrow\ ({\F} 
\NRO_{\pi'})\big)\Big) \;  \land $\\
%
$\hspace{1cm}\Big(({\always} \bigwedge_{a \in \Act_B} a_{\pi} \leftrightarrow 
a_{\pi'} )\ \rightarrow \big(({\F} \NRR_{\pi'}) \leftrightarrow\ ({\F} 
\NRO_{\pi'})\big)\Big)$}\\
\hline
\end{tabular}
\end{center}
%
Observe that trace $\pi$ expresses effectiveness (i.e., an honest behvavior 
of all parties), while trace $\pi'$ is a trace that behaves similarly to 
trace $\pi$ as far as the actions of $\partyA$ or $\partyB$ are concerned 
while ensuring fair receipt of $\NRR$ and $\NRO$. The negated formula for BMC 
is then:

\begin{center}
\centering % used for centering table
\begin{tabular}{ |c|c| } 
\hline
\thead{$\neg$ Fairness} & \thead[l]{ $\neg\varphi_{\fair} = \forall \pi. \exists \pi'.$ 
$\neg \big(({\F} m_{\pi}) \land ({\F} \NRR_{\pi}) \land ({\F}\NRO_{\pi})\big) \lor$ \\
$\hspace{1cm}  \Big(({\always} \bigwedge_{a \in \Act_A} a_{\pi} \leftrightarrow a_{\pi'} )\ \land \neg \big(({\F} \NRR_{\pi'}) \leftrightarrow ({\F} \NRO_{\pi'})\big)\Big) \lor$\\
$\hspace{1cm}  \Big(({\always} \bigwedge_{a \in \Act_B} a_{\pi} \leftrightarrow a_{\pi'} )\ \land \neg \big(({\F} \NRR_{\pi'}) \leftrightarrow ({\F} \NRO_{\pi'})\big)\Big)$}\\
\hline
\end{tabular}
\end{center}

%
In this case study, we evaluate two different models of trusted third party 
from~\cite{jmm11}. 
%
First, we pick an incorrect implementation in~\cite{jmm11}, named 
$T_{\incorrect}$, which $\partyB$ can choose not to send out $\NRR$ after 
receiving $\NRO$.
%
We obtain a SAT result from \HyperQube.
%
The challenge with a SAT result with a $\forall\exists$ formula is that the 
solver understandably does not return an witness.
%
Thus, a SAT result can be either due to non-existence of an effective trace or 
the fact that all conforming traces are unfair.
%
To clarify this, one can verify the protocol with respect to formula 
$\exists \pi. ({\F} m_{\pi} \land {\F} \NRR_{\pi} \land {\F} \NRO_{\pi})$.
%
This step was successful, meaning that an effective trace exists.
%
This means that the original SAT result indicates that the protocol includes an 
unfair trace. 

On the contrary, the implementation named $T_{\correct}$ in~\cite{jmm11}, where 
$T$ always guarantees the message exchange event is fair between the two 
parties, \HyperQube returns UNSAT. This result indicates that all traces in the 
correct system satisfies fairness in non-repudiation. 

%
\textcolor{red}{In this case, both SAT and UNSAT results from $\HyperQube$ can be concluded soundly by two different 
{\em halting} semantics, $\hpes$ and $\hopt$. Since non-repudiation protocol is a terminating system, when we reach the halting state, we draw conclusion based on the observations upto the halting state. That is, using $\hpes$ to consider a SAT result is inferring a counterexample that the given modelviolates the property infinitely, while using $\opt$ to consider an UNSAT result is inferring that no future bad eventuality will happen so the given model satisfy the property.}  
%




\subsection{Case study 5: Privacy-Preserving Path Planning for Robots}
%
In addition to model checking problems, inspired by the work in~\cite{wnp19}, 
we 
also explore other applications that involve hyperproperties with quantifier 
alternation.
%
One such application is searching the optimal solution for robotic planning. 
%
For example, given a map with an initial state and a goal state, the shortest 
path from initial state to goal state is a traces $\pi$, such that $\pi$  can 
reach the goal state and for all other traces $\pi'$, $\pi'$ should not reach 
the goal state until $\pi$ reached it. 
%
In other words, the shortest path is a path on the map that reaches the goal 
state before all other paths did. We express this specification as the 
following hyperproperty:
%

\begin{center}
\centering % used for centering table
\begin{tabular}{ |c|c| } 
\hline
\thead{Shortest Path} & \thead{ $\varphi_{\mathit{sp}} = \exists \pi. \forall 
\pi'. ( \neg \goal_{\pi'}\ \mathcal U\  \goal_{\pi} )$} \\
\hline
\end{tabular}
\end{center}
%
where the atomic proposition $\goal$ denotes that the path has reached the goal 
state.


By enforcing the above formula directly with a map model\todo{BB: Should we 
call it synthesis?}, \HyperQube returns SAT. The returned path represents a 
path that can reach the goal state from the initial state with least steps 
compared to all other paths on the same map. 
%
To further analyze the result, we also consider the terminating bound with 
the formula. 
%
An optimal path searching should terminate when the shortest path is found 
because when a shortest path has been discovered on the map, any further 
exploration will not affect the returning value.


Besides optimal solution searching, HyperLTL also allows us to specify the 
{\em robustness} of paths that are derived by uncertainty in robotic planning. 
%
For example, instead of one single initial state, we now consider a map with a 
set of initial states. 
%
We are interested in a strategy that can help all traces to reach the goal state 
regardless which initial state the path start from. 
%
A robustness strategy searching problem can be presented as follows. 
%
There exists a robust path $\pi$, such that for all paths $\pi'$ starting 
from any initial state, $\pi'$ is able to reach the goal state using the same 
strategy as $\pi$. 
%
Let the notation of $\strategy$ represent a sequential of movements the path 
took (i.e. move up, down, left, or right.). 
%
We write the formula as follows:

\begin{center}
\centering % used for centering table
\begin{tabular}{ |c|c| } 
\hline
\thead{Robustness} & \thead{ $\varphi_{\mathit{rb}} = \exists \pi. \forall 
\pi'.\  {\always}(\strategy_{\pi'} \leftrightarrow \strategy_{\pi}) \rightarrow 
{\F} (\goal_{\pi} \land \goal_{\pi'})$} \\
\hline
\end{tabular}
\end{center}

By enforcing the above formula directly with the map model, \HyperQube returns 
SAT, which indicates that a robustness path has been found. The returned path 
represents a strong strategy that all paths starting from different initial 
state can guarantee of goal reachability using the same strategy. 


\begin{figure}[!htb]
\minipage{0.46\textwidth}
  %\includegraphics[width=\linewidth]{delete_gesture.png}
\centering
\begin{adjustbox}{width=3.3cm}
\begin{tikzpicture}  
    [%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        box/.style={rectangle,draw=gray,thick, minimum size=1cm}, 
    ]%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\foreach \x in {0,1,...,9}{
    \foreach \y in {0,1,...,9}
        \node[box] at (\x,\y){};
}

\node[box,fill=red  ] at (0,0){}; %initial
\node[box,fill=green] at (7,5){};  %goal

%strategy
\draw[arw, ->, line width=0.5mm, color = blue] (0,0) -- (0,1);
\draw[arw, ->, line width=0.5mm, color = blue] (0,1) -- (0,2);
\draw[arw, ->, line width=0.5mm, color = blue] (0,2) -- (0,3);
\draw[arw, ->, line width=0.5mm, color = blue] (0,3) -- (0,4);
\draw[arw, ->, line width=0.5mm, color = blue] (0,4) -- (0,5);
\draw[arw, ->, line width=0.5mm, color = blue] (0,5) -- (0,6);
\draw[arw, ->, line width=0.5mm, color = blue] (0,6) -- (0,7);
\draw[arw, ->, line width=0.5mm, color = blue] (0,7) -- (1,7);
\draw[arw, ->, line width=0.5mm, color = blue] (1,7) -- (2,7);
\draw[arw, ->, line width=0.5mm, color = blue] (2,7) -- (3,7);
\draw[arw, ->, line width=0.5mm, color = blue] (3,7) -- (4,7);
\draw[arw, ->, line width=0.5mm, color = blue] (4,7) -- (5,7);
\draw[arw, ->, line width=0.5mm, color = blue] (5,7) -- (5,6);
\draw[arw, ->, line width=0.5mm, color = blue] (5,6) -- (5,5);
\draw[arw, ->, line width=0.5mm, color = blue] (5,5) -- (6,5);
\draw[arw, ->, line width=0.5mm, color = blue] (6,5) -- (7,5);

%obstacles
\node[box,fill=black] at (5,0){};
\node[box,fill=black] at (7,0){};
\node[box,fill=black] at (3,1){};
\node[box,fill=black] at (9,1){};
\node[box,fill=black] at (1,3){};
\node[box,fill=black] at (3,3){};
\node[box,fill=black] at (6,3){};
\node[box,fill=black] at (3,4){};
\node[box,fill=black] at (5,4){};
\node[box,fill=black] at (6,4){};
\node[box,fill=black] at (7,4){};
\node[box,fill=black] at (1,5){};
\node[box,fill=black] at (3,5){};
\node[box,fill=black] at (4,5){};
\node[box,fill=black] at (8,5){};
\node[box,fill=black] at (1,6){};
\node[box,fill=black] at (2,6){};
\node[box,fill=black] at (3,6){};
\node[box,fill=black] at (4,6){};
\node[box,fill=black] at (6,6){};
\node[box,fill=black] at (7,6){};
\node[box,fill=black] at (8,6){};
\node[box,fill=black] at (1,8){};
\node[box,fill=black] at (2,8){};
\node[box,fill=black] at (3,8){};
\node[box,fill=black] at (1,9){};
\node[box,fill=black] at (2,9){};
\node[box,fill=black] at (4,9){};

\end{tikzpicture}%
\end{adjustbox}%
  
  \caption{Shortest Path}\label{fig:awesome_image1}
\endminipage\hfill
\minipage{0.46\textwidth}
  %\includegraphics[width=\linewidth]{ok_gesture.png}
  \centering
\begin{adjustbox}{width=3.3cm}
\begin{tikzpicture} 
    [%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        box/.style={rectangle,draw=gray,thick, minimum size=1cm}, 
    ]%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\foreach \x in {0,1,...,9}{
    \foreach \y in {0,1,...,9}
        \node[box] at (\x,\y){};
}

%initial states
\node[box,fill=red  ] at (0,0){};
\node[box,fill=red  ] at (1,0){};
\node[box,fill=red  ] at (2,0){};
 
 %goal
\node[box,fill=green] at (6,9){};  
\node[box,fill=green] at (7,9){};  
\node[box,fill=green] at (8,9){};  

%strategy
\draw[arw, ->, line width=0.5mm, color = blue] (2,0) -- (3,0);
\draw[arw, ->, line width=0.5mm, color = blue] (3,0) -- (3,1);
\draw[arw, ->, line width=0.5mm, color = blue] (3,1) -- (4,1);
\draw[arw, ->, line width=0.5mm, color = blue] (4,1) -- (4,2);
\draw[arw, ->, line width=0.5mm, color = blue] (4,2) -- (5,2);
\draw[arw, ->, line width=0.5mm, color = blue] (5,2) -- (5,3);
\draw[arw, ->, line width=0.5mm, color = blue] (5,3) -- (6,3);
\draw[arw, ->, line width=0.5mm, color = blue] (6,3) -- (6,4);
\draw[arw, ->, line width=0.5mm, color = blue] (6,4) -- (6,5);
\draw[arw, ->, line width=0.5mm, color = blue] (6,5) -- (6,6);
\draw[arw, ->, line width=0.5mm, color = blue] (6,6) -- (6,7);
\draw[arw, ->, line width=0.5mm, color = blue] (6,7) -- (7,7);
\draw[arw, ->, line width=0.5mm, color = blue] (7,7) -- (7,8);
\draw[arw, ->, line width=0.5mm, color = blue] (7,8) -- (7,9);
\draw[arw, ->, line width=0.5mm, color = blue] (7,9) -- (8,9);


%obstacles
\node[box,fill=black] at (5,0){};
\node[box,fill=black] at (6,0){};
\node[box,fill=black] at (7,0){};
\node[box,fill=black] at (8,0){};
\node[box,fill=black] at (9,0){};
\node[box,fill=black] at (6,1){};
\node[box,fill=black] at (7,1){};
\node[box,fill=black] at (8,1){};
\node[box,fill=black] at (9,1){};
\node[box,fill=black] at (7,2){};
\node[box,fill=black] at (8,2){};
\node[box,fill=black] at (9,2){};
\node[box,fill=black] at (8,3){};
\node[box,fill=black] at (9,3){};
\node[box,fill=black] at (9,4){};

\node[box,fill=black] at (0,5){};
\node[box,fill=black] at (0,6){};
\node[box,fill=black] at (1,6){};
\node[box,fill=black] at (0,7){};
\node[box,fill=black] at (1,7){};
\node[box,fill=black] at (2,7){};
\node[box,fill=black] at (0,8){};
\node[box,fill=black] at (1,8){};
\node[box,fill=black] at (2,8){};
\node[box,fill=black] at (3,8){};
\node[box,fill=black] at (0,9){};
\node[box,fill=black] at (1,9){};
\node[box,fill=black] at (2,9){};
\node[box,fill=black] at (3,9){};
\node[box,fill=black] at (4,9){};

\end{tikzpicture}
\end{adjustbox}
  \caption{Robust Strategy}\label{fig:awesome_image2}
\endminipage
\end{figure}







\subsection{Case study 6: Generate Mutants in Mutation Testing}
%
Another application of hyperproperty with quantifier alternation is for 
efficiently generating test suite for mutation testing ~\cite{ftw19}
%
We look at the beverage machine model in this paper. 
%
The beverage machine has three possible inputs: {\em request}, {\em fill}, or {\em none}. Based on the input, the machine may output {\em coffee}, {\em tea}, or {\em none}. 
%
We also use an atomic proposition $\mut$ to mark mutated traces, and $\neg\mut$ for non-mutated traces.
% 
In this non-deterministic model, a potentially killable mutants for mutation testing is a mutated trace $\pi$ such that, for all other non-mutated $\pi'$ who have same inputs as $pi$, the outputs will eventually diverge.
%


\begin{center}
\centering % used for centering table
\begin{tabular}{ |c|c| } 
\hline
\thead{Mutant in \\ Non-deterministic Model} & \thead{ $\exists \pi \forall \pi' (\mut_{\pi} \land \neg \mut_{\pi'}) \land \big((\inputt_{\pi} \leftrightarrow \inputt_{\pi'})\ \mathcal U\ (\outputt_{\pi} \not\leftrightarrow \outputt_{\pi'})\big)$} \\
\hline
\end{tabular}
\end{center}
%
\HyperQube returns SAT with the above formula. 
%
The returned path represents a valid mutant for mutation testing. 
%
Our experiment result shows that \HyperQube is able to output a mutant with given formula in a very short amount of time, which provides an efficient solution for test suite generation of mutation testing.




\subsection{Summary Tables}

%
We summarize our results for all case studies. In Table 2., we present the solving time in the right-most column for prove/disprove a property for a given model
%
In Table 3., we present how we map the $\HyperQube$ outputs to a infinite inference for model checking problems. 
%
Table 4. shows the solving time comparison of $\HyperQube$ and the existing model checking tool {\em MCHyper}~\cite{??} with different symmetry property for Lamport's Bakery Algorithm. 
%
Table 5. shows how $\HyperQube$ is more efficient on synthesizing robotic planning strategy in compare with the technique introduced in ~\cite{??}.



\begin{table}[ht]
\caption{Case studies results of BMC for hyperproperties using \HyperQube} % title of Table
\centering % used for centering table
\begin{tabular}{|c |c | c c c c c c c |} 
\hline\hline %inserts double horizontal lines
case\# & Model  & Original $\varphi$ & \#unroll & semantics & QBF result & genqbf [s] & QuAbS [s] & Total [s]  \\ [0.5ex] % inserts table
%heading
\hline\hline % inserts single horizontal line
(case0.1) & \thead{Bakery.3proc} & \thead{ $\forall\forall\ (\sym1)$} & 7 & $\pes$ & SAT  & 0.44 & 0.04 & \textbf{0.48}  \\ 
\hline
(case0.2) &\thead{Bakery.3proc} & \thead{ $\forall\forall\ (\sym2)$} & 12 &  $\pes$ & SAT  & 1.31 & 0.15&  \textbf{1.46}  \\ 
\hline
(case0.3) &\thead{Bakery.3proc} & \thead{ $\forall\forall\ (\sym3)$} & 20 & $\opt$ & UNSAT  & 2.86 & 4.87 & \textbf{7.73}  \\ 
\hline
(case1.1) &\thead{Bakery.3proc} & \thead{ $\varphi_{\sym1}$ } & 10 &  $\pes$ & SAT  & 0.86 & 0.11& \textbf{0.97}  \\ 
\hline
(case1.2) &\thead{Bakery.3proc} & \thead{ $\varphi_{\sym2}$ } & 10 &  $\pes$ & SAT  & 0.76 & 0.17&  \textbf{0.93} \\ 
\hline
(case1.3) &\thead{Bakery.5proc} & \thead{ $\varphi_{\sym1}$} & 10 & $\pes$ & SAT  & 23.57 & 1.08 & \textbf{24.65} \\ 
\hline
(case1.4) &\thead{Bakery.5proc} & \thead{ $\varphi_{\sym2}$} & 10 & $\pes$ & SAT  & 29.92 & 1.43&  \textbf{31.35} \\ 
\hline
(case2.1) &\thead{SNARK-bug1} & $\varphi_{\linearizability}$ & 26 & $\pes$ & SAT & 88.42  &  383.60&  \textbf{472.02}   \\
\hline
(case2.2) &\thead{SNARK-bug2} & $\varphi_{\linearizability}$ & 40 & $\pes$ & SAT & 718.09  &  779.76&  \textbf{1497.85}  \\
\hline
(case3.1) &\thead{3-Thread \\ ({\em incorrect})} &$\varphi_{\NI}$ & 57 & $\hpes$ & SAT & 19.56 & 46.66&  \textbf{66.22}  \\
\hline
(case3.2) &\thead{3-Thread \\ ({\em correct)}} &$\varphi_{\NI}$ & 57 & $\hopt$ & UNSAT & 23.91 & 33.54 & \textbf{57.45}  \\
\hline
(case4.1) &\thead{Non-repudiation \\ Protocol \\ ($T_{\incorrect}$)} & $\varphi_{\fair}$ & 15 & $\hpes$  & SAT & 0.10 & 0.27&  \textbf{0.37} \\
\hline
(case4.2) &\thead{Non-repudiation \\ Protocol \\ ($T_{\correct}$)}& $\varphi_{\fair}$ & 15 & $\hopt$  & UNSAT & 0.08 & 0.12 & \textbf{0.20} \\
\hline\hline
\end{tabular}
\end{table}




\begin{table}[ht]
\caption{Mappings of Cases with Semantics} % title of Table
\centering % used for centering table
\begin{tabular}{|l |c |l |l |l |l |} 
\hline\hline %inserts double horizontal lines
Semantics  & Model & Property & QBF & Infinite Inference & Conclusion   \\ [0.5ex] % inserts table
%heading
\hline\hline
\multirow{2}{*}{$\pes$} 	& \thead{Bakery\\ $\mathit{original}$} &  $\varphi_{\sym}$ 	& SAT & \multirow{2}{*}{\thead[l]{$M \models_k^{\mathit{pes}} \neg \varphi \rightarrow  M \models \neg \varphi$}} & Bakery $\not\models \varphi_{\sym}$ \\\cline{2-4}\cline{6-6}
					& SNARK&  $\varphi_{\linearizability}$ 	& SAT &  & SNARK $\not\models \varphi_{\linearizability}$   \\\hline\hline
${\opt}$ 				&\thead{Bakery\\ $\mathit{contracted}$} &  $\varphi_{\sym}$ 	& UNSAT & \thead[l]{$M \not\models_k^{\mathit{opt}} \neg \varphi \rightarrow  M \not\models \neg \varphi$} & Bakery $\models \varphi_{\sym}$ \\\hline\hline
\multirow{2}{*}{$\bpes$}	& \thead{Non-repudiation \\ protocol \\ ${\mathit{incorrect}}$} 	& $\varphi_{\fair}$ 	& SAT & \multirow{2}{*}{\thead[l]{$M \not\models_k^{\mathit{bpes}} \neg \varphi \rightarrow  M \not\models \neg \varphi$}} & NRP $\not\models$ $\varphi_{\fair}$ \\\cline{2-4}\cline{6-6}
		& \thead{3-Threads \\ $\mathit{incorrect}$}					& $\varphi_{\NI}$   	& SAT &  & 3-Thread $\not\models \varphi_{\NI}$\\\hline\hline
\multirow{2}{*}{$\bopt$}	& \thead{Non-repudiation \\ protocol\\ ${\mathit{correct}}$} 	& $\varphi_{\fair}$ 	& UNSAT & \multirow{2}{*}{\thead[l]{$M \not\models_k^{\mathit{bopt}} \neg \varphi \rightarrow  M \not\models \neg \varphi$}} & NRP $\models$ $\varphi_{\fair}$ \\\cline{2-4}\cline{6-6}
		& \thead{3-Threads \\ $\mathit{correct}$}					& $\varphi_{\NI}$   	& UNSAT &  & 3-Thread $\models \varphi_{\NI}$\\\hline\hline
\multirow{3}{*}{\thead[l]{Synthesis \\ ($\pes$)}} 	& \thead{Robotic} & $\varphi_{\shortest}$ 		& SAT & \multirow{3}{*}{\thead[l]{$M \models_k^{\mathit{pes}} \varphi \rightarrow  M \models \varphi$}} & sortest path exists\\\cline{2-4}\cline{6-6}
		& \thead{Robotic} & $\varphi_{\rub}$ 			& SAT &  & robust path exists\\\cline{2-4}\cline{6-6}
		& \thead{Mutation \\ Testing} & $\varphi_{\mut}$ 			& SAT &  & mutant exists\\
\hline\hline
\end{tabular}
\end{table}


\begin{table}[ht]
\caption{Case studies results of hyperproperties for disproving symmetric property of 
bakery algorithm using \HyperQube, in comparison with the experimental results in ~\cite{??}}  % 
\centering % used for centering table
\begin{tabular}{|c|c| c| c|} 
\hline\hline %inserts double horizontal lines
Model  & Original $\varphi$  & \HyperQube & MCHyper   \\ [0.5ex] % inserts table
%heading
\hline\hline % inserts single horizontal line
\thead{Bakery 3proc} & $\forall\forall\ \sym1$ & 0.48 & 1.36 \\ 
\hline
\thead{Bakery 3proc} & $\forall\forall\ \sym2$ & 1.46 & 16.37 \\ 
\hline\hline
\thead{Bakery 3proc} & $\forall\exists\ \sym1$ & 0.97 &  0.88 (with strategy given) \\ 
\hline
\thead{Bakery 3proc} & $\forall\exists\ \sym2$ & 0.93 &  0.52 (with strategy given) \\ 
\hline
\thead{Bakery 5proc} & $\forall\exists\ \sym1$ & 24.65 & 2.13 (with strategy given)\\ 
\hline
\thead{Bakery 5proc} & $\forall\exists\ \sym2$ & 31.35 & 2.47 (with strategy given)\\ 
\hline\hline
\end{tabular}
\end{table}




\begin{table}[ht]
\caption{Case studies results of hyperproperties for robotic planning using 
\HyperQube, in comparison with the experimental results in ~\cite{cfst19}} 
\centering % used for centering table
\begin{tabular}{|c || c ||  r r  r || r  r  r |} 
\hline\hline %inserts double horizontal lines
  &    \#unroll & gen [s] & Z3 [s] & Total[s] & genqbf [s] & QuAbS [s] & Total [s] \\   [0.5ex]
\hline \hline
\thead{Shortest path \\ $(map\ size:  10^{2})$ } & 20 & 8.31 & 0.33 & \textbf{8.64} & 1.30 & 0.57 & \textbf{1.87}  \\ \hline
\thead{Shortest path \\ $(map\ size:  20^{2})$ } & 40 & 124.66 & 6.41 & \textbf{131.06} & 4.53 & 12.16 & \textbf{16.69}  \\  \hline
\thead{Shortest path \\ $(map\ size:  40^{2})$ } & 80 & 1093.12 & 72.99 & \textbf{1166.11} & 36.04 & 35.75 & \textbf{71.79}  \\  \hline
\thead{Shortest path \\ $(map\ size:  60^{2})$ } & 120 & 4360.75 & 532.11 & \textbf{4892.86} & 105.82 & 120.84 & \textbf{226.66}  \\  \hline
\thead{Initial state robustness \\ $(map\ size:  10^{2})$ } & 20 & 11.14 & 0.45 & \textbf{11.59} & 1.40 & 0.35 & \textbf{1.75}  \\ \hline
\thead{Initial state robustness \\ $(map\ size:  20^{2})$ } & 40 & 49.59 & 2.67 & \textbf{52.26} & 15.92 & 15.32 & \textbf{31.14}  \\  \hline
\thead{Initial state robustness \\ $(map\ size:  40^{2})$ } & 80 & 216.16 & 19.81 & \textbf{235.97} & 63.16 & 20.13 & \textbf{83.29}  \\  \hline
%Generate Mutant & 8 & SAT & 0.01 & 0.02 & a mutant  \\ [1ex] % [1ex] adds vertical space
%\hline %inserts single line
\hline
\end{tabular}
\end{table}






==> code.tex <==
\section{Pseudo-code of Case Studies}

\subsection{Bakery Algorithm}
\begin{algorithm}[H]
\caption{Bakery}
\SetAlgoLined
%\KwResult{How the bakery protocol works}
 init(MAX/ $P_1$.ticket... $P_n$.ticket/ $P_1$.status... $P_n$.status):= 0/ 0...0/ noncrit...noncrit \;
 \While{true}{
 \ForEach{k in 1...n}{
  \uIf{select($P_k$)}{
   	$P_k$.ticket = MAX + 1\;
   	$P_k$.status = wait\;
  	 }
   \uElseIf {$P_k$.status = wait}{
   	\eIf{$P_k$.ticket = min($P_1$.ticket... $P_n$.ticket)}{
		$P_k$.status = crit \;
	}{
		$P_k$.status = wait \;
	}
 }}}
\end{algorithm}

\subsection{SNARK Algorithm}
\begin{algorithm}[H]
\setcounter{AlgoLine}{0}
\caption{SNARK}
\SetAlgoLined
%\KwResult{How the beverage machine works}
 %init(input/ output/ water/ mut):= $\epsilon$/ $\epsilon$/ 2/ \{T, F\} \;
 
 
\SetKwFunction{Fun}{popRight}
\Fun{}{
 \\ \While{true}{
	rh = RightHat\;
	lh = LeftHat\;
	
	\If{rh$\rightarrow$R = rh}{
		return "empty"\;
	}
	\uIf{rh = lh}{
		\If{DCAS($\&$RightHat, $\&$LeftHat, rh, lh, Dummy, Dummy)}{
		return rh $\rightarrow$V;}
	}
   	\uElse{
	rhL = rh$\rightarrow$L\;
   	\If{DCAS($\&$RightHat, $\&$rh$\rightarrow$L, rh, rhL, rhL, rh)}{
		result = rh$\rightarrow$V\;
		rh$\rightarrow$R = Dummy\;
		return result\;
	}
}}}
\SetKwFunction{Fun}{popLeft}
\Fun{}{
 \\ \While{true}{
 	lh = LeftHat\;
	rh = RightHat\;
	\If{lh$\rightarrow$L = lh}{
		return "empty"\;
	}
	\uIf{lh = rh}{
		\If{DCAS($\&$LeftHat, $\&$RigtHat, lh, rh, Dummy, Dummy)}{
		return lh $\rightarrow$V;}
	}
   	\uElse{
	lhR = lh$\rightarrow$R\;
   	\If{DCAS($\&$LeftHat, $\&$lh$\rightarrow$R, lh, lhR, lhR, lh)}{
		result = lh$\rightarrow$V\;
		lh$\rightarrow$L = Dummy\;
		return result\;
	}
}}}
\end{algorithm}

\newpage

\begin{algorithm}[H]
\setcounter{AlgoLine}{38}
\SetKwFunction{Fun}{pushRight}
\Fun{}{
 \\ 
  	nd = new Node()\;
	\If{nd = null}{
		return "full"\;
	}
	nd$\rightarrow$R = Dummy\;
	nd$\rightarrow$V = v\;
	
 	\While{true}{	
	rh = RightHat\;
	rhR = rh$\rightarrow$R\;
	\uIf{rhR = rh}{
		nd$\rightarrow$L = Dummy\;
		lh = LeftHat;
		\If{DCAS($\&$RightHat, $\&$LeftHat, rh, lh, nd, Dummy)}{
		return success\;}
	}
   	\uElse{
	nd$\rightarrow$L = rh\;
   	\If{DCAS($\&$RightHat, $\&$lh$\rightarrow$R, rh, rhR, nd, nd)}{
	        return success\;
	}
}}}
\end{algorithm}


\subsection{Typed Multi-threaded Program}
\begin{algorithm}[H]
\caption{Typed Multi-threaded Program}
\SetAlgoLined
%\KwResult{How the beverage machine works}
 %init(input/ output/ water/ mut):= $\epsilon$/ $\epsilon$/ 2/ \{T, F\} \;
 Thread $\alpha$:\\
 \While{mask != 0 }{
 	\While{trigger0 = 0}{no-op;}
	result = result $\|$ mask ; // bitwise 'or' \\
	trigger0 = 0\;
	maintrigger = matintrigger + 1 \;
	\If{ maintrigger = 1}{
		trigger1 = 1\;
	}
}
Thread $\beta$:\\
 \While{mask != 0 }{
 	\While{trigger1 = 0}{no-op;}
	result = result $\&$ !mask ; // bitwise 'and' \\
	trigger1 = 0\;
	maintrigger = matintrigger + 1 \;
	\If{ maintrigger = 1}{
		trigger0 = 1\;
	}
}
Thread $\gamma$:\\
 \While{mask != 0 }{
 	maintrigger = 0 \;
	\eIf{PIN $\&$ mask = 0} {trigger0 = 1\;}
	{trigger1 = 1\;}
 	\While{maintrigger != 2}{no-op;}
	mask = mask/2\;
}
trigger0 = 1\;
trigger1 = 1\;
\end{algorithm}



\subsection{Typed Multi-threaded Program}
\begin{algorithm}[H]
\caption{Non-repudiation Protocol}
\SetAlgoLined
%\KwResult{How the beverage machine works}
%init(input/ output/ water/ mut):= $\epsilon$/ $\epsilon$/ 2/ \{T, F\} \;
$T_{correct}$:\\
\hspace{0.6cm}(1) skip until A:m$\rightarrow$T \;
\hspace{0.6cm}(2) skip until A:NRO$\rightarrow$T \;
\hspace{0.6cm}(3) T$\rightarrow$B:m \;
\hspace{0.6cm}(4) skip untill B$\rightarrow$T: NRR\;
\hspace{0.6cm}(5) T$\rightarrow$B:NRO\;
\hspace{0.6cm}(6) T$\rightarrow$A:NRR\;


$T_{incorrect}$:\\
\hspace{0.6cm}(1) skip until A:m$\rightarrow$T \;
\hspace{0.6cm}(2) skip until A:NRO$\rightarrow$T \;
\hspace{0.6cm}(3) T$\rightarrow$B:m \;
\hspace{0.6cm}(4) T$\rightarrow$B:NRO\;
\hspace{0.6cm}(5) skip untill B$\rightarrow$T: NRR\;
\hspace{0.6cm}(6) T$\rightarrow$A:NRR\;


\end{algorithm}


==> soundness.tex <==
\section{Soundness Results}
\label{sec:soundness}

In this section, we discuss the soundness of our approach. In particular, 
given a we establish a connection between $\krip \models \varphi$ and 
$\qbf{\krip, \varphi}_k$. We first recall the standard definitions of safety 
and co-safety. In the sequel, for an LTL formula $\varphi$, we denote the 
language of the formula by $\lang(\varphi)$, i.e., the set of all traces that 
satisfy $\varphi$. 

\begin{definition}
\label{def:safety}

We say that an LTL formula $\varphi$ is a {\em safety} property iff
%
\begin{align*}
\forall t \in \alphabet^\omega. t \not \in \lang(\varphi) \; \rightarrow \; 
\Big(\exists m \in \alphabet^*. m \leq t \, \wedge \, \big(\forall t' \in 
\alphabet^\omega. m \leq  t' \rightarrow t' \not \in L(\varphi)\big)\Big)
\end{align*}
%
where `$\leq$' denotes the prefix relation.
\end{definition}
% 
For instance, $\always p$ is a safety formula.

\begin{definition}
\label{def:cosafety}

We say that an LTL formula $\varphi$ is a {\em co-safety} property iff
%
\begin{align*}
\forall t \in \alphabet^\omega. t \in \lang(\varphi) \; \rightarrow \; 
\Big(\exists m \in \alphabet^*. m \leq t \, \wedge \, \big(\forall t' \in 
\alphabet^\omega. m \leq  t' \rightarrow t' \in L(\varphi)\big)\Big)
\end{align*}
%
where `$\leq$' denotes the prefix relation.
\end{definition}
%
For instance, $\F p$ is a co-safety formula.

\subsection{The Alternation-free Fragment}

\subsection{The Safety Fragment}
\label{sec:ae}

\begin{theorem}
\label{thrm:safety}
Let $\varphi = \forall \pi.\exists \pi'.\psi$ and let $k$ be a bound.
%
If $\qbf{\krip, \neg \varphi}_k$ is satisfiable for the pessimistic
unrolling then $\krip \not \models \varphi$.
\end{theorem}

\begin{proof}
 
Suppose that $\qbf{\krip, \neg \varphi}_k$ is satisfiable for some $k \geq 1$. 
This means that there exists some $i \in [0, k]$, such that formula $\neg 
\varphi = \exists \pi.\forall \pi'.\neg \psi$  
 
\end{proof}


\subsection{The Co-safety Fragment}
\label{sec:cosafety}

This fragment is essentially the dual of the fragment discussed in 
Section~\ref{sec:safety}.

\begin{theorem}
\label{thrm:ea-cosafety}
Let $\varphi = \exists \pi.\forall \pi'.\psi$ and $k$ be a bound. If
$\qbf{\krip, \neg \varphi}_k$ is unsatisfiable for the optimistic
unrolling, then $\krip \models \varphi$.


\end{theorem}

\subsection{BMC for Terminating Programs}

